Arithmetic Counts of Tropical Plane Curves and Their Properties

Recently, the first and third author proved a correspondence theorem which recovers the Levine-Welschinger invariants of toric del Pezzo surfaces as a count of tropical curves weighted with arithmetic multiplicities. In this paper, we study properties of the arithmetic count of plane tropical curves satisfying point conditions. We prove that this count is independent of the configuration of point conditions. Moreover, a Caporaso-Harris formula for the arithmetic count of plane tropical curves is obtained by moving one point to the very left. Repeating this process until all point conditions are stretched, we obtain an enriched count of floor diagrams which coincides with the tropical count. Finally, we prove polynomiality properties for the arithmetic counts using floor diagrams.

==> old_introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract and introduction prior to 13. September 2023
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{abstract}
	Tropical plane curves can be used to count rational algebraic plane curves satisfying point conditions both over the complex and over the real numbers. In both cases, we consider the same set of tropical plane curves, depending on the degree and the choice of point conditions. We only vary the multiplicity with which each tropical curve is counted. The arithmetic or quadratically enriched count of plane curves can be specialized to arbitrary fields. The first and third author proved a correspondence theorem in which the tropical count is also enriched via arithmetic multiplicities. When specializing to the complex or real numbers, we obtain the well-known tropical complex resp.\ real multiplicities. In this paper, we study properties of arithmetic counts of plane curves satisfying point conditions by means of tropical geometry, making use of the correspondence theorem. We prove that the count of tropical curves with arithmetic multiplicity is independent of the point conditions. By moving one point to the very left, a Caporaso-Harris formula for the arithmetic count of plane curves satisfying point conditions is obtained. Repeating this process until all point conditions are stretched, we obtain a count of floor diagrams which can also be enriched with arithmetic multiplicities. Finally, we prove polynomiality properties for counts of arithmetic curves using floor diagrams. To sum up, the arithmetic enrichment of the tropical plane curve count interacts nicely with its combinatorics.
\end{abstract}




Enumerative geometry poses geometric counting problems defined over some fixed base field~$K$. Often, $K$ is taken to be the field of complex numbers since this field is algebraically closed, thus leading to desirable properties of the counting problem. For example, consider count of complex plane curves of fixed degree $d$ and genus $g$ passing through some points. This number is a so-called Gromov-Witten invariant of the plane and is denoted $N(d,g)$. It is indeed an invariant in the sense that $N(d,g)$ does not depend on the position of the points, as long as they are chosen generically. In contrast, when we choose $K = \RR$ to count real plane curves satisfying real point conditions, the invariance does no longer hold. For example, there can be $8$, $10$, or $12$ rational real cubics passing through $8$ real points in the plane \cite{DK00}. However, over $\mathbb{R}$ one can often introduce signed counts which are invariant, and where the sign naturally depends on geometric properties of the objects to be counted. In the example of rational plane curves subject to point conditions, Welschinger established an invariant $W(d)$ by counting each curve with a sign taking the number of solitary nodes into account \cite{Wel05}.

The success of tropical methods in enumerative geometry started with Mikhalkin's correspondence theorem~\cite{Mi03}, in which he proved the equality of numbers $N(d,g)$ of complex plane curves of fixed degree and genus satisfying point conditions with their tropical counterparts $N(d, g)^\trop$. Similarly, in the rational case there is also a correspondence theorem expressing the Welschinger invariant $W(d)$ as a tropical count. It is remarkable that the two tropical counts are in fact summing over the same set of tropical curves, but counting them with complex or real multiplicity to obtain the Gromov-Witten or Welschinger invariant.

Since recently, $\mathbb{A}^1$-enumerative geometry offers a universal approach for geometric counting problems valued in the Grothendieck-Witt ring, which can be specialized to any field.
For example, there is an arithmetic count of lines in a cubic surface \cite{KW17}, an arithmetic count of bitangents to a smooth plane quartic curve \cite{LV19}, and an arithmetic count of plane curves satisfying point conditions \cite{LevineWelschinger,KassLevineSolomonWickelgren}.
The tropical approach taken to arithmetic counts of bitangents \cite{MPS22} as well as to B\'ezout's theorem \cite{puentes2022quadratically} reveals how well tropical degenerations interact with arithmetic multiplicities. 

The first and third author proved an enriched correspondence theorem for the count of curves satisfying point conditions \cite{JPP23}. This is not restricted to the case of counting curves in the projective plane $\mathbb{P}^2$, instead we can count curves in any toric surface. A lattice polygon $\Delta$ defines a toric surface as well as a curve class given by hyperplane sections. We denote the count of complex curves of class $\Delta$ and genus $g$ satisfying point conditions by $N(\Delta,g)$. In the case of $\mathbb{P}^2$ and curves of degree $d$ (corresponding to the triangle $\Delta_d$ with vertices $(0,0)$, $(0,d)$ and $(d,0)$), we continue to use the simplified notation $N(d,g)$.

To obtain the arithmetic count of genus $g$ curves of class $\Delta$ satisfying point conditions, denoted by $N_{\mathbb{A}^1}(\Delta,g)$, via tropical geometry, we count each tropical curve $C$ with an arithmetic multiplicity $\mult_{\mathbb{A}^1}(C)$. When specializing to the field of complex numbers, we recover the complex multiplicity of $C$. If the toric surface is a del Pezzo surface and the genus is zero, then specializing to the reals and taking the signature, we obtain the real multiplicity with which $C$ contributes to the Welschinger invariant.

In this paper, we study combinatorial properties of the tropical arithmetic count of plane curves.
We introduce a tropical arithmetic count for any genus and any curve class $\Delta$ in a toric surface, obtaining the numbers $N^{\trop}_{\mathbb{A}^1}(\Delta,g)$. We show that this count is invariant with respect to the point configuration. For genus $0$ and for curves on toric del Pezzo surfaces, the correspondence theorem mentioned above yields the equality of these numbers with the arithmetic count of rational plane curves satisfying point conditions, $N_{\mathbb{A}^1}(\Delta,0)$.


Since the count is invariant, we can move one of our points very far to the left, leading to a further degeneration of tropical plane curves. To use this degeneration in a recursion, we first need to further enlarge our counting problem by allowing ends of higher weight for our tropical curves, corresponding to higher contact orders with the toric boundary. We spell this out for the case of $\mathbb{P}^2$, obtaining a Caporaso-Harris formula \Felix{cite Caporaso Harris and tropical version} which can be used to recursively compute the enriched numbers of rational plane curves satisfying point conditions, $N_{\mathbb{A}^1}(d,0)$. Our proof builds on the tropical proof of the Caporaso-Harris formula in \cite{GM052}.

Applying the step in the Caporaso-Harris recursion until all points are stretched in a small horizontal strip, the tropical curves to be counted can be controlled by even simpler combinatorial objects called floor diagrams \cite{BM08, FM09}. For this purpose, we restrict to Hirzebruch surfaces $\mathbb{F}_k$. The class of a curve in a Hirzebruch surface is denoted by $\Delta_k(a,b)$, see Figure \ref{fig-Hirz}.
We construct an arithmetic count of floor diagrams which equals the tropical numbers $N^{\trop}_{\mathbb{A}^1}(\Delta_k(a,b),g)$, which in case $g=0$ equals the arithmetic count $N_{\mathbb{A}^1}(\Delta_k(a,b),0)$ by the correspondence theorem.

Finally, we use the floor diagram count of arithmetic numbers to prove polynomiality properties. The investigation of such properties goes back to the case of double Hurwitz numbers which count genus $g$ degree $d$ covers of $\mathbb{P}^1$ with two special ramification profiles $\mu,\nu \vdash d$ over $0$ and $\infty$ and only simple ramification else, at fixed points. Goulden, Jackson, and Vakil showed that these numbers are polynomial in the entries $\mu_i,\nu_j$ of the two partitions $\mu,\nu$ \cite{gjv:ttgodhn}, and related this to interesting geometric properties of counts of covers. The piecewise polynomial structure of double Hurwitz numbers can easily be obeserved tropically \cite{cjm:wcfdhn}. The similarity of the count of tropical covers and the count of floor diagrams counting tropical plane curves allowed to apply these tropical methods also to obtain a piecewise polynomial result for counts of curves in Hirzebruch surfaces \cite{AB14}. More precisely, we fix the width $a$ of the polygon in Figure \ref{fig-Hirz}, and we fix the number of left and right ends respectively. We consider the weights $\mu_i$ of the right ends and $\nu_j$ of the left ends as variables, where $\nu$ is a partition of $b$ and $\mu$ of  $ ak+b$. Then the complex count of tropical curves (and with it, via the correspondence theorem, the complex count) can be viewed as a function in the variables $\mu_i,\nu_j$. As the arithmetic multiplicity can be viewed as an interpolation between the complex and real count, one can deduce also piecewise polynomiality properties of the arithmetic count.
